Heuristics for Selecting Predicates for Partial Predicate Abstraction

In this paper we consider the problem of configuring partial predicate abstraction that combines two techniques that have been effective in analyzing infinite-state systems: predicate abstraction and fixpoint approximations. A fundamental problem in partial predicate abstraction is deciding the variables to be abstracted and the predicates to be used. In this paper, we consider systems modeled using linear integer arithmetic and investigate an alternative approach to counter-example guided abstraction refinement. We devise two heuristics that search for predicates that are likely to be precise. The first heuristic performs the search on the problem instance to be verified. The other heuristic leverages verification results on the smaller instances of the problem. We report experimental results for CTL model checking and discuss advantages and disadvantages of each approach.

==> implementation.tex <==

We have chosen the Action Language Verifier (ALV) \cite{YB09} to combine predicate abstraction and fixpoint approximations. ALV is an infinite-state model checker that can analyze transition systems defined over boolean and unbounded integer domains for CTL properties. It uses BDD representation for the boolean domain and supports two alternative representations for the integer domain: polyhedra based representation and automata based representation. ALV leverages the widening operator defined by the underlying integer representations to compute over-approximations for the fixpoint computations of $EU$, $AU$, $EF$, $AF$ operators (-A flag) and the set of reachable states (-F flag). 

We extended ALV with predicate abstraction (-PA flag) by transforming the original Kripke structure according to Definition \ref{def:abstractingKripke} based on a set of predicates provided as input. The CTL property is transformed by traversing the abstract syntax tree of the property and computing the abstraction on the propositional formula using the abstraction function $\alpha$ given in Section \ref{sec:approach}. 
%The implementation also provides the concretized abstract temporal property to the user to make sure that the property that is inferred to hold in the concrete system matches what the user 
%intended to verify. It is important to note that the exact transformation of the property depends on the set of predicates and it helps to user to understand the real implications of abstract model checking, i.e., whether the property in its original property can be assumed to hold.

We would like to note that we did not incorporate a counter-example guided abstraction refinement (CEGAR) loop to ALV as comparing a CEGAR loop based predicate abstraction with fixpoint approximations is outside the scope of this paper. We wanted to find out whether combining predicate abstraction with fixpoint approximation has any benefits when the set of predicates can be easily extracted from the model.

Unlike traditional implementation of predicate abstraction, our approach to generation of the abstract transition system does not involve weakest precondition computation with respect to the predicates. Also, our approach does not use an SMT solver, in the traditional sense, to compute the abstraction. This is because we literally perform the existential quantification in Equations \ref{eq:alpha} and \ref{eq:alphaT} using ALV's  polyhedral symbolic representation that uses the Omega Library \cite{omega}. However, in our approach the price is paid by having a  blow-up in the abstract transition system that is exponential in the number of predicates. We deal with this blow-up by using the simplification heuristic of ALV \cite{YB02f}.

%In our approach the abstract model may have some unbounded concrete variables, whose behavior from the concrete model is preserved exactly. The state-space exploration of those variables can be subject to fixpoint approximations through approximate reachable set computation, temporal operator computation, or both. The soundness of the approximate computations have been discussed in Section \ref{sec:approach}. 

==> proofSketch.tex <==
Let $p_1$ and $p_2$ be two predicates that are not compatible, i.e., when $\varphi={p_1,p_2}$ we cannot show that $T \models \phi$. 

Show that  adding a predicate $p_3$ such that $V_{p_3} \intersect (V_{p_1} \cup V_{p_2}) = \emptyset$ does not improve the precision. 

Lemma A: Given $(\alpha,\gamma)$ is a Galois connection, $a \wedge b \not = false$ implies $\alpha(a) \wedge \alpha(b) \not = false$.

Lemma G: Show existence of a Galois connection between   
partially abstracted domain $\{p_1,p_2\}$ and partially abstracted domain $\{p_1,p_2,p_3\}$ through $\alpha_{\{p_3\}$  when $V_{p_3} \intersect (V_{p_1} \cup V_{p_2}) = \emptyset$: 
$\exists V_{p_3}. (\exists V_{p_1}.V_{p_2}. s \wedge (p_1 \iff b_1) \wedge (p_2 \iff b_2)) \wedge (p_3 \iff b_3)= \exists V_{p_3}.V_{p_1}.V_{p_2}. s \wedge (p_1 \iff b_1) \wedge (p_2 \iff b_2) \wedge (p_3 \iff b_3)$. This allows incremental abstraction while keeping a Galois connection. The goal, however, is not to optimize abstraction, rather, show that when two predicates are compatible adding predicates on new variables does not improve the precision.

Lemma H: Given $\alpha_{\{p_1,p_2\}}(I) \wedge EF(\alpha_{\{p_1,p_2\}}(\neg \phi)) \not = false$ then $\alpha_{\{p_1,p_2,p_3\}}(I) \wedge EF(\alpha_{\{p_1,p_2,p_3\}}(\neg \phi)) \not = false$ by considering various cases of the number of iterations for least fixpoint computation for both parts. 

Cases: a) assume that $EF(\alpha_{\{p_1,p_2\}}(\neg \phi)) = abs_1(\neg \phi))$ and $EF(\alpha_{\{p_1,p_2,p_3\}}(\neg \phi)) = abs_2(\neg \phi))$ (follows from Lemma G and Lemma A).

$abs_1(s)$ means $\alpha_{\{p_1,p_2\}}(s)$ and $abs_2(s)$ means $\alpha_{\{p_1,p_2,p_3\}}(s)$.

b) $EF(\alpha_{\{p_1,p_2\}}(\neg \phi) = abs_1(\neg \phi)$  and $EF(\alpha_{\{p_1,p_2,p_3\}}(\neg \phi)) = Z_K$.  Follows from Lemma G and Lemma A that $abs_2(I) \wedge  abs_2(\neg \phi) \not = false$, which implies that $I_{abs2} \wedge EF( \alpha_{\{p_1,p_2,p_3\}}(\neg \phi)) \not = false$ as $abs_2(\neg \phi) \rightarrow EF(abs_2(\neg \phi))$.

c) $EF(\alpha_{\{p_1,p_2\}}(\neg \phi) = Z_K$  and $EF(\alpha_{\{p_1,p_2,p_3\}}(\neg \phi)) = abs_2(\neg \phi)$. Assume $k$ is the smallest k such that $I \wedge (abs_1(\neg \phi) \vee \bigvee_{j=1}^{k}Pre^j(abs_1(\neg phi))) \not = false$.  From Lemma A and the fact that $\alpha((abs_1(\neg \phi) \vee \bigvee_{j=1}^{k}Pre^j(abs_1(\neg phi)))) \equiv \alpha(\neg abs_1) \vee \bigvee_{j=1}^{k}\alpha(Pre_1(\neg \phi_1)) \rightarrow abs_2(\neg phi) \vee \bigvee_{j=1}^{k} \vee \bigvee_{j=1}^{k} Pre_2(\neg \phi_2))$. This is because $\alpha(Pre(\neg \phi_1)) = \exists p_3. \exists V'_1. T_1 \wedge \phi'_1 \wedge (p_3 \iff b_3)$, $Pre_2(\\neg \phi_2) = \exists V_2'. (\exists p_3. T_1 \wedge (p_3 \iff b)) \wedge (\exists p_3. \neg \phi'_1  \wedge (p_3 \iff b_3))$. Since the existential quantification on $p_3$ is applied to the transition relation and the atomic formula separately in $Pre_2(\\neg \phi_2)$, $\alpha(Pre(\neg \phi_1)) \rightarrow  
Pre_2(\neg \phi_2)$. 

$I \wedge Pre^k(abs_1(\neg phi)) \not = false$ implies $I \wedge \exists p_3. Pre^k(abs_1(\neg phi)) \not = false$ as $f \rightarrow \exists x. f$ and $a \wedge b \not = false$ and $b \rightarrow B$ implies $a \wedge B \not = false$. $Pre_{abs}^k(a_{abs}) = \exists V'. T_{abs} \wedge \exists V'. T_{abs} \wedge \exists V'. T_{abs} ... \wedge a_{abs}$. 
Since $EF(\alpha_{\{p_1,p_2,p_3\}}(\neg \phi)) = abs_2(\neg \phi)$, we can rewrite abs_2(\neg \phi) as $Pre_{abs_2}^k(abs_2(\neg \phi))$. By intorudcing $\exists p_3

Since $\exists x. f_1 \wedge f_2 \implies \exists x. f_1 \wedge \exists x. f_2$, 
($\exists p_3$ a short hand for $\exists V_{p_3}$.

d) $EF(\neg \alpha_{\{p_1,p_2\}}\phi) = Z_{K_1}$ and EF(\alpha_{\{p_1,p_2,p_3\}}(\neg \phi)) = Z_{K_2}$.
d.1 ) $K_1 < K_2$: d.2) ...
No need for induction. Considering all cases is sufficient. 

So if two predicates are incompatible adding a new predicate on a different set of variables does not improve the precision.

A relevant result is that if two predicates are compatible adding a new predicate on a different set of variables and incompatible with one of the predicates would hurt the precision.




Compute a set of scores for each property of interest. Combine all to find those that are compatible in most of the properties to leverage common construction time 

$compat(p_i) = | \{ p_j \ | \ 0 \leq j \leq N \wedge j \not = i \wedge Abstract(I,S,R,\{p_i,p_j\}) \models \varphi \} |$

$scope(p_i) = | \{ scope(p_j) \ | \ 0 \leq j \leq N \wedge j \not = i \wedge Abstract(I,S,R,\{p_i,p_j\}) \models \varphi \} |$

